Distributed System Contract Monitoring

The use of behavioural contracts, to specify, regulate and verify systems, is particularly relevant to runtime monitoring of distributed systems. System distribution poses major challenges to contract monitoring, from monitoring-induced information leaks to computation load balancing, communication overheads and fault-tolerance. We present mDPi, a location-aware process calculus, for reasoning about monitoring of distributed systems. We define a family of Labelled Transition Systems for this calculus, which allow formal reasoning about different monitoring strategies at different levels of abstractions. We also illustrate the expressivity of the calculus by showing how contracts in a simple contract language can be synthesised into different mDPi monitors.

==> eptcsdata.tex <==
\providecommand{\firstpage}{23}
\providecommand{\publicationstatus}{E. Pimentel, V. Valero (Eds.): Workshop on Formal Languages\\
and Analysis of Contract-Oriented Software 2011 (FLACOS'11)\\
EPTCS 68, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.68.4}{10.4204/EPTCS.68.4}}
\pdfoutput=1

